Using Waste Factor to Optimize Energy Efficiency in Multiple-Input Single-Output (MISO) and Multiple-Input Multiple-Output (MIMO) Systems

This paper introduces Waste Factor (W) and Waste Figure (WF) to assess power efficiency in any multiple-input multiple-output (MIMO) or single-input multiple-output (SIMO) or multiple-input single-output (MISO) cascaded communication system. This paper builds upon the new theory of Waste Factor, which systematically models added wasted power in any cascade for parallel systems such as MISO, SIMO, and MIMO systems, which are prevalent in current wireless networks. Here, we also show the advantage of W compared to conventional metrics for quantifying and analyzing energy efficiency. This work explores the utility of W in assessing energy efficiency in communication channels, within Radio Access Networks (RANs).

==> deleted.tex <==


% \section{Advantage of Waste Factor Compared to Other Power Efficiency Metrics}

% \textit{W} provides a clear and quantifiable measure of power efficiency for a RAN chain, contrasting with traditional energy efficiency metrics such as Power Added Efficiency (PAE) for power amplifiers and conventional Energy Efficiency (EE) for cellular networks.

% Power-added efficiency (PAE) is defined as \cite{PAE1983}:
% \begin{equation}
%     PAE = \frac{P_{out} - P_{in}}{P_{dc}},
% \end{equation}
% where \(P_{out}\) is the output power, \(P_{in}\) is the input power, and \(P_{dc}\) is the DC power consumed. PAE measures the efficiency of power addition in amplifiers relative to the DC power used.

% Energy Efficiency (EE), on the other hand, is defined as the ratio of the utility function (such as capacity, throughput, or spectral efficiency) to the total power consumed. For illustration purposes, we choose Shannon capacity \cite{ShannonCapacity} as the utility function, then EE is given by:
% \begin{equation}
%     EE = \frac{R}{P_{total}},
% \end{equation}
% where \(R\) represents the network throughput (e.g., data rate) and \(P_{total}\) is the total power consumption.

% Comparatively, the Waste Factor offers several advantages compared to conventional power efficiency metrics:

% \begin{itemize}

% \item \textbf{Flexibility and Comprehensiveness}: \textit{W} is a versatile metric that provides a clear and comprehensive analysis of power efficiency in various systems, including cellular networks, data centers, and cascaded devices. It encompasses signal path, non-signal path, and non-path power consumption, offering a holistic view of power waste and total power consumption.

% \item \textbf{Channel and System-Specific Efficiency}: \textit{W} excels in evaluating power efficiency in wired or wireless scenarios by considering channel characteristics, losses, and $W$ of individual components in cascaded and parallel systems (e.g., MISO, SIMO, MIMO). This enables accurate assessments of overall system performance and identifies bottlenecks in power efficiency.

% \item \textbf{Optimization and Comparative Analysis}: By breaking down power efficiency at component and stage levels, \textit{W} facilitates the identification of specific areas for improvement, enables targeted optimizations, and provides a standardized metric for comparing power efficiency across different devices, systems, or network configurations. This fosters innovation and drives the development of energy-efficient communication systems.

% \item \textbf{Integration into System Design}: Incorporating \textit{W} into the design process allows engineers to make informed decisions about component selection, system architecture, and power management strategies from the early stages of development, leading to more sustainable and energy-efficient communication systems.


% \end{itemize}
